Minimizing Age in Gateway Based Update Systems

We consider a network of status updating sensors whose updates are collected and sent to a monitor by a gateway. The monitor desires as fresh as possible updates from the network of sensors. The gateway may either poll a sensor for its status update or it may transmit collected sensor updates to the monitor. We derive the average age at the monitor for such a setting. We observe that increasing the frequency of transmissions to the monitor has the upside of resetting sensor age at the monitor to smaller values. However, it increases the length of time that elapses before a sensor is polled again. This motivates our investigation of policies that fix the number of sensors s the gateway polls before transmitting to the monitor. For any s, we show that when sensor transmission times to the gateway are independent and identically distributed (iid), for independent but possibly non-identical transmission times to the monitor, it is optimal to poll a sensor with the maximum age at the gateway first. Also, under simplifying assumptions, the optimal value of s increases as the square root of the number of sensors. For non-identical sensor transmission times, we consider a policy that polls a sensor such that the resulting average change in age is minimized. We compare our policy proposals with other policies, over a wide selection of transmission time distributions.

==> conclusions.tex <==
\section{Conclusions}
\label{sec:conclusions}

==> related.tex <==
\section{Related Work}
\label{sec:related}
The Age of information (AoI) in multiple systems has been studied as a scheduling problem, and the problem explored in the current work also resembles the same. The authors in
\cite{AoI-Igor-SPBN,AoI-BN-RA,SA-BN-nb} presented the problem of minimizing the AoI in a wireless broadcast network, where \cite{AoI-Igor-SPBN} presented low complexity algorithms for general networks and the \cite{AoI-BN-RA, SA-BN-nb} developed an online and offline Markov Decision Process (MDP) scheduling, and an index algorithm exploiting the structure of the problem with buffer and no buffer case respectively. 

The use of AoI as a metric has recently been used in energy harvesting servers used for sending \textit{time-stamped} updates of a single source sensor to a destination node \cite{OS-AoI-EHS, SS-MAoI-EHS, AoI-ERC}. The work presented in \cite{AoI-ERC}, shows that the knowledge of expected value of the current age and the energy level of the server leads to a threshold policy, minimizing the average age as well as the peak age for an arbitrary energy replenishment profile. Similarly, in \cite{SS-MAoI-EHS} the author uses the prior information to develop a threshold policy so as to minimize the AoI for a unit battery case. In contrast the authors in \cite{OS-AoI-EHS} developed different heuristic for infinite, finite and unit energy level of the server to minimize the long term average AoI, further proving optimality for the infinite case. For a given fixed policy where the source updates enter service if idle, \cite{AoI-Igor-SPBN} analyses the average AoI when servers can simultaneously service and harvest energy and otherwise for infinite and finite battery case.

Minimizing the AoI has also been studied under the context of link scheduling in a wireless system \cite{OLS-MM-PAOI, OFI-LS}. The maximum peak age of information is minimized using a fast scheduling algorithm in \cite{OLS-MM-PAOI}. In \cite{OFI-LS} a number of links with a common channel is considered and a scheduling algorithm is developed capable of handling scalability of the network.  

%The realm of AoI scheduling policies have influenced many system and one of its first applications was witnessed in data warehouses \cite{S-SS-DW, SU-RTSW}. The authors in \cite{S-SS-DW} introduced \textit{staleness} and \textit{strench} as two of the metrics in minimizing the age of the updates, and on the assumption of sufficiently fast processors, develop an online non-preemptive algorithm to minimize the same. The work in \cite{SU-RTSW} focus on developing an online scheduling algorithm in minimizing staleness of the table. 

Minimizing the AoI of multi-source system has been recently studied by \cite{AO-STS-MSS}, where only one source can be scheduled to the destination node via a channel. The objective was to minimize total average peak age (TaPa) and total average age (TaA) of the sources. The use of separation principle was used to develop an optimal scheduling and optimal sampling strategy. Furthermore, the use of approximate Bellman's equation was used to develop an optimal sampler to minimize the TaA. The work presented in \cite{AO-STS-MSS} closely resembles the current system in terms of the network topology, however the current work does deviates from the \textit{generate at will} model and assume random arrival rate from the sources. 


==> rl.tex <==
\section{Dynamic Programming}
The current problem can be defined in a Dynamic Programming (DP) form similar to \cite{AoI-Igor-SPBN}. 
